Towards Robust Multi-tab Website Fingerprinting

Website fingerprinting enables an eavesdropper to determine which websites a user is visiting over an encrypted connection. State-of-the-art website fingerprinting (WF) attacks have demonstrated effectiveness even against Tor-protected network traffic. However, existing WF attacks have critical limitations on accurately identifying websites in multi-tab browsing sessions, where the holistic pattern of individual websites is no longer preserved, and the number of tabs opened by a client is unknown a priori. In this paper, we propose ARES, a novel WF framework natively designed for multi-tab WF attacks. ARES formulates the multi-tab attack as a multi-label classification problem and solves it using the novel Transformer-based models. Specifically, ARES extracts local patterns based on multi-level traffic aggregation features and utilizes the improved self-attention mechanism to analyze the correlations between these local patterns, effectively identifying websites. We implement a prototype of ARES and extensively evaluate its effectiveness using our large-scale datasets collected over multiple months. The experimental results illustrate that ARES achieves optimal performance in several realistic scenarios. Further, ARES remains robust even against various WF defenses.

==> section/5-data-collection.tex <==
\section{Data Collection}
\label{sec:data_collection}

To the best of our knowledge, there are no publicly available multi-tab website fingerprint datasets. Most prior WF studies collected their datasets under the unrealistic single-tab browsing settings~\cite{rimmer2018automated, sirinam2018deep}. 
To accurately evaluate the effectiveness of \ours in the real world, we collect our Tor browsing datasets under the real multi-tab scenario.
In particular, we develop an automatic Tor browsing tool based on the Tor browser and the Selenium framework~\cite{selenium} by using over 1,000 lines of code (LOC).
We deploy our tool on \xinhao{40} different cloud servers located in different regions to simulate Tor clients located across the globe.
\xinhao{Our data collection is divided into two phases from May 2021 to December 2021 and from June 2022 to November 2022.}
%Our data collection lasts from May 2021 to December 2021. 
Similar to the existing study~\cite{wang2013improved}, the Tor browser is set to visit websites without caching. To avoid noise interference, we stop all other processes running on the cloud servers to prevent generating background traffic. 

In general, our data collection tool takes the following steps to repeatedly collect each multi-tab Tor browsing session: 
(i) Start the tcpdump tool for network traffic collection and open the Tor browser; 
(ii) Open multiple browser tabs sequentially to visit different websites;
(iii) We use the tcpdump tool to collect the entire stream of packets generated while visiting the websites and record them into a pcap file;
(iv) Close the Tor browser and its relevant processes to clean the browser's profile information after a pre-defined browsing time; 
(v) Close the tcpdump tool and regard the collected pcap file as the traffic instance of this session; 
(vi) Wait for 15 seconds, check all flows of this session are terminated, and then start a new iteration. By applying the steps above, we can ensure that a pcap file associated with a session only contains the traffic of websites browsed in this session.
Afterward, we extract the direction sequence of packets from each pcap file as the feature vector used for WF attacks. A traffic segment means a subsequence of the entire direction sequence. Specifically, we collect various sessions by opening different numbers of browser tabs in closed and open-world scenarios. The number of browser tabs is set from two to five. Also, the interval between loading two consecutive websites in one session is randomly selected between 3 and 10 seconds. 
Note that, prior art~\cite{gong2020zero} shows that the front packets contain most website-specific information and are sufficient to construct WF attacks. Thus, we set the browsing time of each session as 240 seconds which, according to our measurement study, is long enough to load the entire pages for most websites.

Note that, our data collection does not incur negative impacts on the real-world Tor network or other Tor clients. We only launch and collect about 1,500 browsing sessions per day, a tiny fraction of all the sessions created by millions of real Tor clients each day~\cite{tormetrics}.
Further, we only collect the browsing sessions launched by ourselves locally such that our datasets do not contain other Tor clients' data.


\noindent \textbf{Multi-tab Datasets.}
We collect multi-tab datasets in closed and open-world scenarios. In the closed-world scenario,  clients will only visit a small set of monitored websites. 
For \xinhao{a} fair comparison, we use the same settings as prior arts~\cite{rimmer2018automated, sirinam2018deep}, \ie we choose Alexa's top 100 websites as the set of monitored websites. Under the closed-world \emph{k}-tab setting, we randomly select \emph{k} websites from this monitored set as website combinations. For each website combination, our tool visits the homepage of the websites in the combination sequentially with random intervals. Meanwhile, our tool collects the website traffic as an instance of this combination. Since the total number of website combinations becomes extremely large as \emph{k} increases, \eg there are over 76 million 5-tab combinations for 100 monitored websites, we only randomly generate thousands of website combinations for each \emph{k}-tab setting and each combination will be collected for 20 times, \ie a combination has 20 instances.

In the open-world scenario, clients can visit other websites outside the monitored websites set. Therefore, we build a non-monitored website set from Alexa’s top 20,000, excluding the first 100 websites used in the closed-world scenario. Under the open-world \emph{k}-tab setting, we randomly select \emph{k}-1 websites from the monitored websites set and one website from the non-monitored set as the website combinations. Note that, in the open-world scenario, each monitored website is associated with one specific label, and all non-monitored websites are associated with same single label different from all monitored websites. 
Thus, we only have to select one non-monitored website for each \emph{k}-tab open-world website combination. Besides, each website in the non-monitored set will be selected only once. Thus, the open-world website combinations under a specific tab setting will have different non-monitored websites. Then, our tool uses the same procedures \xinhao{for} closed-world scenarios to collect the traffic instances for these combinations. Due to the significant number of open-world website combinations, each combination will only be collected once. 

We further check all collected instances to ensure the quality of our datasets. First, we examine the relevant Selenium logs, to remove the generated error instances, \eg website server timeouts or Selenium crashes. Second, at the end of one browsing session, our tool saves a screenshot for each browsed website such that we can easily filter out the instances containing failed website browsing. After these two steps, we only keep the closed-world website combinations having at least 10 instances. 
%The number of collected closed and open-world instances \xinhao{is} shown in Table~\ref{tab:datasets}.

\noindent \textbf{Defense datasets.} 
% We generate defense datasets by converting the multi-tab datasets according to the state-of-the-art WF defenses. 
Since most heavyweight WF defenses cannot be applied to the real-world Tor network due to their high latency overheads\footnote{As pointed out by the guideline of the Tor project, WF defenses having latency overhead may cause out-of-memory errors on the Tor relay nodes}~\cite{gong2020zero}, in our experiments, we choose two representative lightweight defenses, \ie WTF-PAD~\cite{juarez2015wtf} and Front~\cite{gong2020zero}, and a heavyweight defense, \ie Tamaraw~\cite{cai2014tamaraw}. WTF-PAD and Front only inject packets in the traffic (\ie incurring data overheads) and will not delay data packets. Tamaraw introduces high latency and data overheads, but it is effective against the existing WF attacks~\cite{sirinam2018deep,rahman2019tik,gong2020zero}. 
\xinhao{
We collect a 2-tab defense dataset for each chosen defense setting with real-world defense deployment in the Tor network based on WFDefProxy~\cite{gong2021wfdefproxy}.
With WFDefProxy, we can implement each defense as a pluggable transport (PT) that obfuscates the traffic between the client and the entry node in the real world.}
%We convert all 2-tab instances based on the released WF defenses codes~\cite{gong2020zero} to generate a defense dataset for each chosen defense setting. 
Besides, we generate another defense dataset by randomly inserting dummy packets \xinhao{in the traffic}. Random inserting is a common defense strategy in practice. To avoid incurring high data overheads, the percentage of dummy packets per instance is limited to 20\%. Thus, we obtain four defense datasets and each dataset includes \xinhao{20 thousand 2-tab} instances. Each network traffic instance in the defense datasets corresponds to a multi-tab browsing session perturbed by a specific defense setting. 

\noindent \textbf{Datasets for Dynamic Settings.} 
Most of the existing studies assume that an adversary learns the number of tabs a priori.
In practice, it is difficult to obtain such information.
In addition, since the  clients may change their deployed WF defense over time, the deployed WF defense may be also transparent to the adversary. Thus, we consider dynamic settings where the number of tabs and deployed WF defenses are unknown. To generate evaluation datasets for such dynamic settings, we randomly sample the traffic instances from the multi-tab and defense datasets under different settings and mix them together. 
In particular, we create two sets of datasets for the dynamic settings: the dynamic multi-tab datasets and the dynamic defense datasets. In the former set, we randomly select and mix 100k closed-world instances and 20k open-world instances with different numbers of tabs, where the 2-tab instances account for 40\%, 3-tab instances account for 30\%, 4-tab instances account for 20\%, and 5-tab instances account for 10\%. 
\xinhao{In the latter set, 60k instances collected with WF defenses are randomly selected and mixed}. We select the same number of instances from the four types of defenses (Random instances, WTF-PAD instances, Front instances, and Tamaraw instances). 

\noindent \textbf{Datasets for Beyond Alexa-top 100 Websites.} 
The available public WF datasets~\cite{rimmer2018automated,sirinam2018deep} are all based on Alexa-top websites. This may have two potential problems. 
% \first These websites are biased. 
\first Alexa-top websites are ranked solely based on the number of visits, without considering other factors like the types of websites. For example, the Alexa-top 100 websites include a large number of search websites and social networking websites. 
% \second Deviation of the websites from the dark web. 
\second The Alexa-top websites do not include the websites of the dark web which Tor users may visit. 
To address this problem, we collect a dataset for a more representative list of websites. We first select 10 websites from the dark web which are anonymized using the Onion service.
%These websites contain various types of drug dealing, arms trafficking, gambling, etc. 
For ethical reasons, we only visit the home page and collect traffic for research purposes, and do not publish links. 
Then we select 9 types of websites including search websites, social networking websites, video websites, news websites, e-commerce websites, etc., and choose 10 websites from each type. %as the list of websites for our data collection.
% We collected 58 thousand samples for this experiment.

\noindent \textbf{Datasets for Multiple Tor Browser Versions.} 
We consider a practical scenario where multiple Tor browser versions co-exist. 
In contrast to the existing work~\cite{juarez2014critical} that uses three Tor browser versions, we select five Tor browser versions released in the last two years, including version \texttt{10.0.15}, \texttt{10.5}, \texttt{11.0.3}, \texttt{11.0.10}, and \texttt{11.5}.
We use more recent Tor Browsers because older versions are vulnerable to fingerprinting attacks. Before version \texttt{10.0.15}, a lot of effort was made to implement traffic padding and fix a series of bugs~\cite{torversion,torrelease}.
We deploy clients in 20 different locations, each of which randomly selects one Tor browser version and accesses websites in 5 tabs. 
%We collect 56 thousand samples in this experiment. 

\noindent \textbf{Datasets for Subpage Browsing.} 
Previous WF attacks~\cite{rimmer2018automated, sirinam2018deep, sirinam2019triplet, panchenko2016cumul,rahman2019tik} are evaluated by assuming that the client only visits the homepage of each website. This is not realistic. We thus consider the case where clients can visit subpages of a website beyond the homepage. To this end, we first collect 1000 subpages of Alexa-top 100 websites based on crawlers and 10 subpages per website. Then each time a client visits the website, a subpage of the website is randomly selected for browsing. 
%We collected 56 thousand of samples for the experiment.

\noindent \textbf{Datasets for Vantage Points.} 
As discussed in Section~\ref{sec:threat_model}, potential adversaries include local network administrators, Internet Service Providers (ISP), and eavesdroppers on the local network. Therefore, the vantage points for deploying WF attacks can vary. 
To evaluate \ours in this scenario, we set up 10  clients and 10 private bridges. 
% While the client browses websites, we randomly collect traffic on the client or on a bridge.
When a client browses websites, it connects to a randomly selected bridge, and then we collect traffic at the bridge. %In total, we collected 53 thousand samples for the experiment.

\noindent \textbf{Datasets generated by Real Users.} 
Finally, we collect browsing traffic generated based on the browsing behavior of real users.
We recruited 50 volunteers from our university, and we provide a wide range of websites (including news, online shopping, social activities, academic activities, etc) for volunteers.  
We record the websites they visited, the number of tabs they opened, and the time interval between two tabs. 
%Volunteers' browsing behavior mainly includes browsing news, online shopping, social activities, academic activities, etc. In particular, volunteers can only browse the list of websites we provide.
We collect 10 testing samples (each sample represents one browsing session) for each user, where the largest number of opened tabs in each session is 20.
In particular, we do not collect or handle any Personal Identifiable Information (PII). The collected trace will not leak the privacy of volunteers.



